Two-User Erasure Interference Channels with Local Delayed CSIT

We study the capacity region of two-user erasure interference channels with local delayed channel state information at the transmitters. In our model, transmitters have local mismatched outdated knowledge of the channel gains. We propose a transmission strategy that only relies on the delayed knowledge of the {\it outgoing} links at each transmitter and achieves the outer-bound for the scenario in which transmitters learn the entire channel state with delay. Our result reveals the subset of the channel state information that affects the capacity region the most. We also identify cases in which local delayed knowledge of the channel state does not provide any gain over the zero knowledge assumption. To do so, we revisit a long-known intuition about interference channels that as long as the marginal distributions at the receivers are conserved, the capacity remains the same. We take this intuition and impose a certain spatial correlation among channel gains such that the marginal distributions remain unchanged. Then we provide an outer-bound on the capacity region of the channel with correlation that matches the capacity region when transmitters do not have access to channel state information.

==> CornerPointP.tex <==
We now provide the achievability strategy for the corner point
\begin{align}
\label{eq:CornerPointAppendix}
\left( R_i, R_{\bar{i}} \right) = \left( \min\left\{ p, pq(1+q)\right\}, p \right) \raisebox{2pt}{.}
\end{align}
It suffices to prove the achievability for $i = 1$.

To achieve this corner point, new challenges arise which are due to the asymmetry of the rates. In this case, ${\sf Tx}_2$ (the primary user) communicates at the full rate of $p$ while ${\sf Tx}_1$ (the secondary user) communicates at a lower rate and tries to coexist with the primary user. In fact ${\sf Tx}_1$ has to take more responsibility in dealing with interference at {\it both} receivers. The proposed transmission strategy consists of three phases as described below. 

We assume that ${\sf Tx}_1$ has $\min\{1,q(1+q)\}m$ bits to communicate while ${\sf Tx}_2$ has $m$ bits. We show that all bits can be delivered in $p^{-1}m + \mathcal{O}\left( m^{2/3} \right)$ time instants with vanishing error probability as $m \rightarrow \infty$. This immediately implies the achievability of the corner point given in (\ref{eq:CornerPointAppendix}).

\noindent {\bf Phase 1}: This phase is similar to Phase 1 of the achievability of the optimal sum-rate point. The main difference is due to the fact that the transmitters have unequal number of bits at the start. In Phase $1$, ${\sf Tx}_1$ (the secondary user) transmits all its initial bits while ${\sf Tx}_2$ (the primary user) only transmits a fraction of its initial bits. Transmitter two postpones the transmission of its remaining bits to Phase 2.

At the beginning of the communication block, we assume that each transmitter has $\min\{1,q(1+q)\}m$ bits in queue $Q_{i \rightarrow i}$ (the initial state of the bits), $i=1,2$. At each time instant $t$, ${\sf Tx}_i$ sends out a bit from $Q_{i \rightarrow i}$, and this bit will either stay in the initial queue or a transition to one of the following possible queues will take place according to the description in Table~\ref{Table:View2}. If at time instant $t$, $Q_{i \rightarrow i}$ is empty, then ${\sf Tx}_i$, $i=1,2$, remains silent until the end of Phase 1.

Phase~$1$ continues for 
\begin{align}
\frac{\min\{1,q(1+q)\}}{1-q^2}m + m^{\frac{2}{3}}
\end{align}
time instants, and if at the end of this phase, either of the queues $Q_{i \rightarrow i}$ is not empty, we declare error type-I and halt the transmission.

Assuming that the transmission is not halted, let $N_{i,1}$ and $N_{i, 2}$, $i=1,2$, denote the number of bits in queues $Q_{i,1}$ and $Q_{i,2}$ respectively at the end of Phase~$1$. The transmission strategy will be halted and an error type-II will occur, if any of the following events happens.
\begin{align}
% \label{eq:errortypeII}
& N_{i,1} > \mathbb{E}[N_{i,1}] + 2 m^{\frac{2}{3}} \overset{\triangle}= n_{i,1}, \quad i=1,2; \nonumber \\
& N_{i,2} > \mathbb{E}[N_{i,2}] + 2 m^{\frac{2}{3}} \overset{\triangle}= n_{i,2}, \quad i=1,2.
\end{align}

From basic probability, we have
\begin{align}
% \label{eq:expectedvalues}
\mathbb{E}[N_{i,1}] = \frac{p^2\min\{1,q(1+q)\}m}{1-q^2},~\mathbb{E}[N_{i,2}] = \frac{pq\min\{1,q(1+q)\}m}{1-q^2}.
\end{align}
At the end of Phase $1$, for $i=1,2$, we add $0$'s (if necessary) in order to make queues $Q_{i,1}$ and $Q_{i,2}$ of size equal to $n_{i,1}$ and $n_{i,2}$ respectively.

Since channel gains are distributed independently, statistically a fraction of $q$ of the bits in $Q_{i,1}$ and a fraction of $q$ of the bits in $Q_{i,2}$ are known to ${\sf Rx}_{\bar{i}}$, $i=1,2$. Denote the number of bits in $Q_{i,j}$ known to ${\sf Rx}_{\bar{i}}$ by
\begin{align}
N_{i,j|{\sf Rx}_{\bar{i}}}, \qquad i,j \in \{ 1, 2 \}.
\end{align}
At the end of communication, if we have
\begin{align}
N_{i,j|{\sf Rx}_{\bar{i}}} < q n_{i,j} - m^{\frac{2}{3}}, \qquad i,j \in \{ 1, 2 \},
\end{align}
we declare error type-III.

Moreover, we note that statistically for every $p^{-1}$ bits in $Q_{\bar{i},1}$, a bit in $Q_{i,1}$ or $Q_{i,2}$ was transmitted simultaneously with one of them. Denote the number of bits in $Q_{i,1}$ or $Q_{i,2}$ that were transmitted simultaneously with a bit in $Q_{\bar{i},1}$ by
\begin{align}
N_{i \rightarrow \bar{i},1}, \qquad i = 1, 2.
\end{align}
At the end of communication, if we have
\begin{align}
N_{i \rightarrow \bar{i},1} < p n_{i,1} - m^{\frac{2}{3}}, \qquad i = 1, 2,
\end{align}
we declare error type-IV. Note that transmitters cannot detect error type-III or error type-IV, but receivers have sufficient information to do so. 

Using the Bernstein inequality, we can show that the probability of errors of types I, II, III, and IV decreases exponentially with $m$. For the rest of this subsection, we assume that Phase~1 is completed and no error has occurred.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent {\bf Phase 2} [transmission of new bits vs interference management]: If $1-\min\{ 1, q(1+q) \} = 0$, then skip Phase~2. In this phase, the primary user ${\sf Tx}_2$ transmits its remaining initial bits while the secondary user ${\sf Tx}_1$ tries to resolve as much interference as it can and deliver some of its bits in $Q_{1,1}$. To do so, the secondary user sends some of its bits in $Q_{1,1}$ at a rate low enough such that both receivers can decode and remove them regardless of what the primary transmitter does. Note that $pq$ of the time, each receiver obtains an interference-free signal from the secondary transmitter, hence, the secondary transmitter can take advantage of these time instants to deliver its bits during Phase~2. 

\begin{table*}[t]
\caption{Transition of the bits from $Q_{2 \rightarrow 2}$ during Phase~2.}
\centering
\begin{tabular}{| c | c | c | c | c | c |}
\hline
case ID		 & channel realization    & state transition  & case ID		 & channel realization    & state transition \\
					 & at time instant $n$    &                   & 					 & at time instant $n$    &                  \\ [0.5ex]
\hline

\raisebox{30pt}{$1$}    &    \includegraphics[height = 2.5cm]{FiguresPDF/ICBTx2.pdf}     &  \raisebox{30pt}{$a \rightarrow Q_{1,1}$}  &  \raisebox{18pt}{$3$}    &    \includegraphics[height = 2.5cm]{FiguresPDF/ICATx2.pdf}     &   \raisebox{18pt}{$a \rightarrow Q_{1 \rightarrow F}$} \\

\hline

\raisebox{30pt}{$2$}    &    \includegraphics[height = 2.5cm]{FiguresPDF/ICCTx2.pdf}     &  \raisebox{30pt}{$a \rightarrow Q_{1,2}$} &  \raisebox{18pt}{$4$}    &    \includegraphics[height = 2.5cm]{FiguresPDF/ICD.pdf}     &   \raisebox{18pt}{$a \rightarrow Q_{1 \rightarrow 1 }$} \\

\hline

\end{tabular}
\label{Table:View2Corner}
\end{table*}

Transmitter ${\sf Tx}_1$ creates a matrix $\mathbf{C}_{1,1}$ of size 
$$\left( pq\frac{1-\min\{ 1, q(1+q) \}m}{1-q^2}+m^{2/3} \right) \times \left( p^2\frac{\min\{1,q(1+q)\}m}{1-q^2} + 2 m^{\frac{2}{3}} \right),$$ 
where the entries of this matrix are drawn from i.i.d. $\mathcal{B}(0.5)$ distribution. We assume that this matrix is generated prior to communication and is shared with receivers. Then ${\sf Tx}_1$ multiplies matrix $\mathbf{C}_{1,1}$ and $Q_{1,1}$. Using point-to-point erasure code of rate $pq$, transmitter ${\sf Tx}_1$ encodes bits $\mathbf{C}_{1,1} Q_{1,1}$ and communicates them during Phase~2. We note that due to the chosen rate (\emph{i.e.} $pq$) as $m \rightarrow \infty$, each receiver can decode bits $\mathbf{C}_{1,1} Q_{1,1}$ with vanishing error probability.

Transmitter ${\sf Tx}_2$ places its remaining $\left(1-\min\{ 1, q(1+q) \} \right)m$ bits in queue $Q_{2 \rightarrow 2}$ (the initial state of the bits). At each time instant $t$ of Phase~2, ${\sf Tx}_2$ sends out a bit from $Q_{2 \rightarrow 2}$, and this bit will either stay in the initial queue or a transition to a new queue will take place according to the description in Table~\ref{Table:View2Corner}. Note that here, since the signal of ${\sf Tx}_1$ can be decoded first, we simply consider the bits of ${\sf Tx}_2$ that were transmitted in case $1$ (see Table~\ref{Table:View2Corner}) to be delivered. At the end of Phase~2, we update the value of $n_{2,2}$ as
\begin{align}
n_{2,2} = \left[ \frac{pq\min\{1,q(1+q)\}}{1-q^2} +  pq\frac{1-\min\{ 1, q(1+q) \}}{1-q^2}\right] m + 3 m^{\frac{2}{3}}.
\end{align}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In this phase, our goal is to empty $Q_{1,2}$. 

\noindent {\bf Phase 3} [encoding and mixing interfering bits]: Transmitter ${\sf Tx}_1$ creates two matrices: $\mathbf{C}_{1,2}$ of size 
$$\left( \frac{p^2\min\{1,q(1+q)\}m}{1-q^2} -  pq\frac{1-\min\{1,q(1+q)\}m}{1-q^2} + 2 m^{\frac{2}{3}} \right) \times \left( \frac{p^2\min\{1,q(1+q)\}m}{1-q^2} + 2 m^{\frac{2}{3}} \right),$$ 
and $\mathbf{C}_{1,3}$ of size 
$$\left( \frac{pq\min\{1,q(1+q)\}m}{1-q^2} + 2 m^{\frac{2}{3}} \right) \times \left( \frac{pq\min\{1,q(1+q)\}m}{1-q^2} + 2 m^{\frac{2}{3}} \right),$$ 
where entries to each matrix are drawn from i.i.d. $\mathcal{B}(0.5)$ distribution. We assume that the matrices are generated prior to communication and are shared with receivers. 

Transmitter ${\sf Tx}_1$ creates
\begin{align} 
\tilde{Q}_{1,1} = \mathbf{C}_{1,2} Q_{1,1}, \nonumber\\
\tilde{Q}_{1,2} = \mathbf{C}_{1,3} Q_{1,2}. 
\end{align}
Then ${\sf Tx}_1$ encodes bits in $\tilde{Q}_{1,1}$ using a point-to-point erasure code of rate $pq$ denoted by $\hat{Q}_{1,1}$ and encodes bits in $\tilde{Q}_{1,2}$ using a point-to-point erasure code of rate $p$ denoted by $\hat{Q}_{1,2}$. Transmitter ${\sf Tx}_1$ communicates\footnote{$,^3$ The two sequences are not of equal length, we can simply add deterministic number of zeros to $\hat{Q}_{1,2}$ to make the two sequences of equal length} $\hat{Q}_{1,1} \oplus \hat{Q}_{1,2}$ during Phase~3.


At the same time, transmitter ${\sf Tx}_2$ creates two matrices: $\mathbf{C}_{2,1}$ of size 
$$\left(  \frac{qp^2\min\{1,q(1+q)\}m}{1-q^2} + 2 m^{\frac{2}{3}} \right) \times \left( \frac{p^2\min\{1,q(1+q)\}m}{1-q^2} + 2 m^{\frac{2}{3}} \right),$$ 
and $\mathbf{C}_{2,2}$ of size 
\begin{align*}
\left( \frac{pq}{1-q^2} m + 3 m^{\frac{2}{3}} \right) \times \left( \frac{pq}{1-q^2} m + 3 m^{\frac{2}{3}} \right),
\end{align*} 
where entries to each matrix are drawn from i.i.d. $\mathcal{B}(0.5)$ distribution. We assume that the matrices are generated prior to communication and are shared with receivers.

% \begin{align*}
% & \left( \left[ \frac{pq\min\{1,q(1+q)\}}{1-q^2} +  pq\frac{1-\min\{ 1, q(1+q) \}}{1-q^2}\right] m + 3 m^{\frac{2}{3}} \right) \times \\
%& \left( \left[ \frac{pq\min\{1,q(1+q)\}}{1-q^2} +  pq\frac{1-\min\{ 1, q(1+q) \}}{1-q^2}\right] m + 3 m^{\frac{2}{3}} \right),
%\end{align*} 


Transmitter ${\sf Tx}_2$ creates
\begin{align} 
\tilde{Q}_{2,1} = \mathbf{C}_{2,1} Q_{2,1}, \nonumber\\
\tilde{Q}_{2,2} = \mathbf{C}_{2,2} Q_{2,2}. 
\end{align}
Then ${\sf Tx}_2$ encodes bits in $\tilde{Q}_{2,1}$ using a point-to-point erasure code of rate $pq$ denoted by $\hat{Q}_{2,1}$ and encodes bits in $\tilde{Q}_{2,2}$ using a point-to-point erasure code of rate $p$ denoted by $\hat{Q}_{2,2}$. Transmitter ${\sf Tx}_2$ communicates$^3$ $\hat{Q}_{2,1} \oplus \hat{Q}_{2,2}$ during Phase~3.

\noindent {\bf Decoding}: Upon completion of the third phase, we show that each receiver has gathered enough linear equations to decode all bits in $Q_{1,1}, Q_{1,2}$ and $Q_{2,2}$. Receiver ${\sf Rx}_i$ first removes the known bits from $Q_{\bar{i},1}$ and $Q_{\bar{i},2}$, $i=1,2$.

Then, each receiver has 
\begin{align*}
& \underbrace{\left( pq\frac{1-\min\{ 1, q(1+q) \}m}{1-q^2} + 2 m^{\frac{2}{3}} \right)}_{\mathbf{C}_{1,1} Q_{1,1}}  \\
& + \underbrace{\left( \frac{p^2\min\{1,q(1+q)\}m}{1-q^2} -  pq\frac{1-\min\{1,q(1+q)\}m}{1-q^2} + 2 m^{\frac{2}{3}} \right)}_{\mathbf{C}_{1,2} Q_{1,1}} \\
& = \frac{p^2\min\{1,q(1+q)\}m}{1-q^2} + 4 m^{\frac{2}{3}}
\end{align*}
randomly generated equations of 
$\frac{p^2\min\{1,q(1+q)\}m}{1-q^2} + 2 m^{\frac{2}{3}}$ 
bits in $Q_{1,1}$. Thus, both receivers can recover the bits in $Q_{1,1}$ with vanishing error probability as $m \rightarrow \infty$. Similarly, receivers have sufficient information to recover bits in $Q_{1,2}$ and $Q_{2,2}$ 

As opposed to other states, not all bits in $Q_{2,1}$ are provided to the receivers by ${\sf Tx}_2$. However, transmitter ${\sf Tx}_2$ is not required to provide all bits in $Q_{2,1}$ to both receivers. The reason is that, once $Q_{1,1}$ and $Q_{1,2}$ are known at the receivers, statistically a fraction $p$ of the bits in $Q_{2,1}$ can be reconstructed at each receiver. Therefore, transmitter ${\sf Tx}_2$ needs to provide a fraction $q$ of the bits in $Q_{2,1}$ to the receivers. We chose the size of $\mathbf{C}_{2,1}$ in Phase~3 accordingly.

We therefore conclude that each receiver can recover its intended bits with vanishing error probability as $m \rightarrow \infty$ in a total of
\begin{align}
\frac{1}{p}m+\mathcal{O}\left( m^{2/3} \right)
\end{align}
time instants.

Hence, if we let $m \rightarrow \infty$, the decoding error probability goes to zero exponentially, and we achieve rate-tuple 
\begin{align}
\left( R_1, R_2 \right) = \left( \min\left\{ p, pq(1+q)\right\}, p \right) \raisebox{2pt}{.}
\end{align}

Similarly, we can achieve the corner point
\begin{align}
\left( R_1, R_2 \right) = \left( p, \min\left\{ p, pq(1+q)\right\} \right) \raisebox{2pt}{.}
\end{align}
Together with the results of Section~\ref{Section:FullGain}, we conclude that $\mathcal{C}\left( \text{V.}8 \right)$ is achievable with local delayed CSIT of View V.2.

==> Remarks.tex <==
In this section, our goal is to provide a better understanding of the converse techniques presented in this paper. To that end, we first describe the converse with global delayed CSIT and then, we highlight the salient techniques that allow us to obtain the outer-bound for local delayed CSIT of Views V.1, V.3, and V.4. The capacity region of the two-user Binary Fading IC with global delayed CSIT was obtained in~\cite{AlirezaBFICDelayed}. The key converse idea there is an extremal entropy inequality for a binary broadcast channel with delayed CSIT.

\subsection{An Extremal Entropy Inequality}

Consider a broadcast setting in which a single-antenna transmitter is connected to two single-antenna receivers through binary fading channels as in Fig.~\ref{Fig:BCDelayed}. For this network, suppose $G_1[t]$ and $G_2[t]$ are distributed as i.i.d. Bernoulli RVs (\emph{i.e.} $G_i[t] \overset{d}\sim \mathcal{B}(0.5)$), $i=1,2$. Then the observed signals are given as
\begin{align}
Y_i[t] = G_i[t] X[t], \qquad i = 1,2,
\end{align}
where $X[t]$ is the transmit signal at time $t$. We assume that at time $t$, the transmitter has access to $\left( G_1[\ell], G_2[\ell] \right)_{\ell=1}^{t-1}$ (delayed CSIT).

The goal is to find the minimum value of $\beta$ in this channel that satisfies
\begin{align}
\label{Eq:Extremal}
H\left( Y_2^n | G^n \right) \geq \beta H\left( Y_1^n | G^n \right).
\end{align}
In a sense, the goal is to quantify how much the transmitter can favor receiver one over receiver two in terms of the available entropy.

\begin{figure}[ht]
\centering
\includegraphics[height = 3.5cm]{FiguresPDF/Portion.pdf}
\caption{A transmitter connected to two receivers through binary fading channels..\label{Fig:BCDelayed}}
\end{figure}

\begin{lemma}[Entropy Leakage~\cite{AlirezaBFICDelayed}]
\label{Lemma:Leakage}
For the channel described above with delayed CSIT and for \emph{any} input distribution, the minimum value of $\beta$ satisfying (\ref{Eq:Extremal}) is $\frac{2}{3}$.
\end{lemma}

\begin{remark}
The lower-bound $\beta = \frac{2}{3}$ is in fact achievable using a simple transmission strategy and thus, the bound is tight in the Entropy Leakage Lemma. Furthermore, to achieve this lower-bound, the transmitter only needs to have access to delayed knowledge of {\it one} of the channel gains {\it not} both. 
\end{remark}

\subsection{Deriving the Outer-Bound and Remarks}

Here, for completeness, we provide the proof of
\begin{align}
R_1 + \frac{3}{2} R_2 \leq \frac{9}{8},
\end{align}
as given in~\cite{AlirezaBFICDelayed} for the two-user BFIC with global delayed CSIT. Suppose the rate tuple $\left( R_1, R_2 \right)$ is achievable. Then we have
\begin{align}
n &\left( R_1 + \beta^{-1} R_2 \right) = H(W_1|W_2, G^n) + \beta H(W_2|G^n) \nonumber \\
& \overset{(\mathrm{Fano})}\leq I(W_1;Y_1^n|W_2,G^n) + \beta I(W_2;Y_2^n|G^n) + n \epsilon_n \nonumber \\
& = H(Y_1^n|W_2,G^n) - \underbrace{H(Y_1^n|W_1,W_2,G^n)}_{=~0} \nonumber \\
& \quad + \beta^{-1} H(Y_2^n|G^n) - \beta^{-1} H(Y_2^n|W_2,G^n) + n \epsilon_n \nonumber \\
& = \beta^{-1} H(Y_2^n|G^n) + H(Y_1^n|W_2,X_2^n,G^n) - \beta^{-1} H(Y_2^n|W_2,X_2^n,G^n) + n \epsilon_n \nonumber \\
& = \beta^{-1} H(Y_2^n|G^n) + H(G_{11}^nX_1^n|W_2,X_2^n,G^n) - \beta^{-1} H(G_{12}^nX_1^n|W_2,X_2^n,G^n) + n \epsilon_n \nonumber \\
& \overset{(a)}= \beta^{-1} H(Y_2^n|G^n) + H(G_{11}^nX_1^n|W_2,G^n) - \beta^{-1} H(G_{12}^nX_1^n|W_2,G^n) + n \epsilon_n \nonumber \\
& \overset{(b)}= \beta^{-1} H(Y_2^n|G^n) + H(G_{11}^nX_1^n|G^n) - \beta^{-1} H(G_{12}^nX_1^n|G^n) + n \epsilon_n \nonumber \\
& \overset{\textrm{Lemma}~\ref{Lemma:Leakage}}\leq \beta^{-1} H(Y_2^n|G^n) + n \epsilon_n \leq \frac{9}{8}n  + n \epsilon_n.
\end{align}
where $(a)$ holds since $X_2^n$ is a deterministic function of $W_2$ and $G^n$; $(b)$ follows from
\begin{align}
\label{eq:addX2}
& 0 \leq H(G_{11}^nX_1^n|G^n) - H(G_{11}^nX_1^n|W_2,G^n) = I\left( G_{11}^nX_1^n; W_2|G^n\right) \nonumber \\
& \quad \leq I\left( W_1,G_{11}^nX_1^n; W_2|G^n\right) = \underbrace{I\left( W_1 ; W_2|G^n\right)}_{=~0 \mathrm{~since~W_1 \perp W_2 \perp G^n}} + \underbrace{I\left( G_{11}^nX_1^n; W_2| W_1, G^n\right)}_{=~0 \mathrm{~since~X_1^n=f_1(W_1,~G^n)}} = 0,
\end{align}
which implies $H(G_{11}^nX_1^n|G^n) = H(G_{11}^nX_1^n|W_2,G^n)$, and similarly $H(G_{12}^nX_1^n|G^n) = H(G_{12}^nX_1^n|W_2,G^n)$. Dividing both sides by $n$ and let $n \rightarrow \infty$, we get
\begin{align}
R_1 + \frac{3}{2} R_2 \leq \frac{9}{8}.
\end{align}

\begin{remark}
As stated above, in order to achieve the lower-bound $\beta = \frac{2}{3}$, a transmitter only needs to have access to delayed knowledge of one of the channel gains {\it not} both. In local delayed CSIT of Views V.1, V.3, and V.4, transmitter ${\sf Tx}_i$ can in fact achieve favor receiver $i$ over receiver $\bar{i}$ in terms of the available entropy by the value given in the Entropy Leakage Lemma ($\beta = \frac{2}{3}$). Thus, to obtain a tight outer-bound, we had to create a spatial correlation among channel gains such that: $(1)$ the capacity region is preserved; and $(2)$ in the new channel with correlated links, a transmitter can no longer favor a receiver to the other. This goal was achieved by setting
\begin{align}
\tilde{G}_{ii}[t] = \tilde{G}_{i\bar{i}}[t] \quad i=1,2.
\end{align}
Then, we were able to show that under such spatial correlation, the capacity region coincides with that of no CSIT (View V.0).
\end{remark}

==> myDefinitions.tex <==


\newcommand*{\MonoPath}{mono}
\newcommand*{\RobPath}{robustness}
\newcommand*{\OutPath}{outer}

\graphicspath{{}{figs/}{../}{../figs/}{../Monograph/monograph/nowformat/}}

\newif\ifmonograph
\monographfalse

\bibliographystyle{plain}
%\bibliographystyle{IEEEbib}

\renewcommand{\caption}[1]{\singlespacing\hangcaption{#1}\normalspacing}
\renewcommand{\topfraction}{0.85}
\renewcommand{\textfraction}{0.1}
\renewcommand{\floatpagefraction}{0.75}


%\usepackage[colorlinks=true,pdfstartview=FitV,linkcolor=black,citecolor=black,urlcolor=blue,plainpages=false]{hyperref}
%
\usepackage[numbers,sort&compress]{natbib}
\renewcommand{\bibfont}{\footnotesize}
%
%
%\usepackage[T1]{fontenc}
%\usepackage[latin1]{inputenc}
%
%%% Math Packages %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\iint\relax
\let\iiint\relax
\let\iiiint\relax
\let\idotsint\relax
\usepackage{amsmath}
%\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{dsfont}
\usepackage{mathrsfs}


%%\usepackage{appendix}
%\usepackage{stfloats}
%
%
%% If the IEEEtran.cls has not been installed into the LaTeX system files,
%% manually specify the path to it:
%% \documentclass[conference]{../sty/IEEEtran}
%\usepackage[]{authblk}
%\usepackage{times}
%\usepackage{epsf}
%\usepackage{psfrag}
%\usepackage{epsfig}
%
%
%\usepackage{amssymb}
%\usepackage{amstext}
%\usepackage{latexsym}
%\usepackage{color}
%\usepackage{ifthen}
%%\usepackage{mycaptions}
%\usepackage{multirow}
%
%\usepackage{subfigure}

\renewcommand{\L}{{\mathcal L}}

\newcommand{\1}{{\bf 1}}
\newcommand{\Z}{{\mathds Z}}
\newcommand{\dis}{{\mathsf{dis}} \,}
\newcommand{\ep}{\epsilon}
\newcommand{\vep}{\varepsilon}

\newcommand{\A}{{\mathcal A}}
\newcommand{\B}{{\mathcal B}}
\newcommand{\C}{{\mathcal C}}

\newcommand{\G}{{\mathcal G}}
\renewcommand{\H}{{\mathcal H}}
\newcommand{\D}{{\mathcal D}}
%\newcommand{\Dr}{{\mathscr D}}

\newcommand{\Dr}{\mathcal{DR}}
%\newcommand{\dof}{\mathscr{D}}
\newcommand{\dof}{\mathbf{D}}
\newcommand{\Dreg}{\dof}


\newcommand{\E}{{\mathcal E}}
\newcommand{\V}{{\mathcal V}}
\renewcommand{\S}{{\mathcal S}}
\newcommand{\I}{{\mathcal I}}
\newcommand{\M}{{\mathcal M}}
\newcommand{\N}{{\mathcal N}}
\newcommand{\U}{{\mathcal U}}
\newcommand{\T}{{\mathcal T}}
\newcommand{\IN}{{\mathbb N}}
\newcommand{\R}{{\mathbb R}}
\newcommand{\Rs}{{\mathcal R}}
\newcommand{\Os}{{\mathcal O}}
\newcommand{\Ps}{{\mathcal P}}
\newcommand{\K}{{\mathcal K}}
\newcommand{\W}{{\mathcal W}}
\newcommand{\X}{{\mathcal X}}
\newcommand{\Y}{{\mathcal Y}}
\newcommand{\F}{{\mathds F}}
\newcommand{\dE}{D_\Sigma}
\newcommand{\q}[2]{Q_{s_{#1},d_{#2}}}
\newcommand{\p}[2]{P_{s_{#1},d_{#2}}}
\newcommand{\m}[2]{M_{s_{#1},d_{#2}}}
\newcommand{\z}[2]{Z_{s_{#1},d_{#2}}}
\newcommand{\ttt}{3 \times 3 \times 3}
\newcommand{\kkk}{K \times K \times K}
\newcommand{\kk}[1]{#1 \times #1 \times #1}
\newcommand{\cT}{{\cal T}}
\newcommand{\cR}{{\cal R}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cC}{{\cal C}}


\newcommand{\s}{{\bf s}}
\renewcommand{\r}{{\bf r}}
\newcommand{\x}{{\bf x}}
\newcommand{\y}{{\bf y}}

\newcommand{\din}{\Delta_{\rm in}}
\newcommand{\dout}{\Delta_{\rm out}}

\newcommand{\bw}{\bar w}
\newcommand{\dbw}{\bar{\bar w}}

\newcommand{\lcrit}{\ell_{\rm crit}}

\newcommand{\lacrit}{\tilde \ell_{\rm crit}}

\newcommand{\loverl}{\ell_{\rm overlap}}

%\newcommand{\corr}{\text{corr}}

\newcommand{\kkkl}[1]{K \hspace{-#1mm} \times \hspace{-#1mm} K \hspace{-#1mm} \times \hspace{-#1mm} K}

\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}

\newcommand{\Vgcs}{V}
\newcommand{\Egcs}{E}

\newcommand{\Zeff}{N}
\newcommand{\Nnoise}{Z}

\newcommand{\vecwc}[1]{{\bf #1}}

\newcommand{\rdecsymb}{a}

\newcommand{\skl}{\vspace{4mm}}

\newcommand{\bfcomment}[1]{ \vspace{3mm}

\noindent {\bf !! -- #1 -- !!}

\vspace{3mm}
}

%\newcommand{\bfcomment}[1]{}  %%% replace by above if draft

\newcommand{\non}{\nonumber \\}

\newcommand{\Ht}{{\mathcal H^{(t)}}}

\newcommand{\IDFT}{\text{IDFT}}
\newcommand{\DFT}{\text{DFT}}

\newcommand{\til}{\tilde}
\renewcommand{\ge}{\gamma}

\newcommand{\MC}[3]{#1\leftrightarrow #2 \leftrightarrow #3}

\newcommand{\fMC}[4]{#1\leftrightarrow #2 \leftrightarrow #3 \leftrightarrow #4}

%\newcommand{\defi}{{\stackrel{\rm \Delta}{\hspace{2mm}=\hspace{2mm}}}}
\newcommand{\defi}{\triangleq}

\newcommand{\error}{\text{\rm error}}

\newcommand{\ol}{\overline}
\newcommand{\ul}{\underline}

\newcommand{\avg}{{\rm avg}}

\newcommand{\bv}{\bf}

\newcommand{\dist}{\phi}

\newcommand{\qd}{\xi}

\newcommand{\Remark}{\noindent \emph{Remark:}\;}

\newcommand{\goesto}{\rightarrow}

\newcommand{\one}{\mathds 1}

\newcommand{\concat}{\oplus}

\newcommand{\SNR}{\text{SNR}}

\newcommand{\vectil}[1]{{\bf \tilde #1}}

%\newcommand{\interf}{\hspace{1mm}{\stackrel{I}{\leadsto}}\hspace{1mm}}
\newcommand{\interf}{\leadsto}
\newcommand{\dinterf}{\hspace{1mm}{\stackrel{I}{\rightarrow}}\hspace{1mm}}

%\newcommand{\st}{\hspace{1mm}|\hspace{1mm}}
\newcommand{\st}{:}

\newcommand{\pr}{$^\prime$}

\newcommand{\cut}{\Omega}
\newcommand{\cutb}{\Theta}

\newcounter{constcount}
\setcounter{constcount}{0}

\newcommand{\resconstcount}{\setcounter{constcount}{0}}

\newcommand{\fref}[1]{Fig.~\ref{#1}}
\newcommand{\eref}[1]{(\ref{#1})}
\newcommand{\tref}[1]{Theorem~\ref{#1}}

\newcommand{\cons}{\stepcounter{constcount} \kappa_{\arabic{constcount}}}
\newcommand{\curcons}{\kappa_{\arabic{constcount}}}

\newcounter{numcount}
\setcounter{numcount}{1}

\newcommand{\eqnum}{\stackrel{(\roman{numcount})}{=}\stepcounter{numcount}}

\newcommand{\leqnum}{\stackrel{(\roman{numcount})}{\leq\;}\stepcounter{numcount}}

\newcommand{\geqnum}{\stackrel{(\roman{numcount})}{\geq\;}\stepcounter{numcount}}

\newcommand{\cnt}{$(\roman{numcount})$ \stepcounter{numcount}}

\newcommand{\rescnt}{\setcounter{numcount}{1}}

\newcommand{\deriv}{$(ii)$\;}

\newcommand{\nueff}{\tilde \nu}

\newcommand{\rank}{{\rm rank}}

%\renewcommand{\vec}[1]{{\bf #1}}

\newcommand{\bvec}[1]{{\bf #1}}

\newcommand{\eq}[1]{(\ref{#1})}

\newcommand{\tr}{^{\dagger}}

%\newtheorem{claim}{Claim}[chapter]

\newcounter{thmcnt}
\setcounter{thmcnt}{0}
%\newcommand{stsec}{\stepcounter{thmcnt}}

  \let\Oldsection\section
%   \makeatletter
%   \renewcommand{\section}{\@startsection{section}{1}{0mm}
%   {\baselineskip}%
%   {\baselineskip}{\normalfont\normalsize\scshape\centering}}%
%   \makeatother  
  
\renewcommand{\section}{\stepcounter{thmcnt}\Oldsection}

\newenvironment{lemmarep}[1]{\noindent {\bf Lemma #1.}\begin{it}}{\end{it}}

\newenvironment{theoremrep}[1]{\noindent {\bf Theorem #1.}\begin{it}}{\end{it}}

\newenvironment{claimrep}[1]{\noindent {\bf Claim #1.}\begin{it}}{\end{it}}

\newenvironment{correp}[1]{\noindent {\bf Corollary #1.}\begin{it}}{\end{it}}

\allowdisplaybreaks


%--------------- Various \newtheorem Declarations -----------------------


\newtheorem{theorem}{Theorem} %[chapter] %[thmcnt]%[section]
\newtheorem{lemma}{Lemma} %[chapter]
\newtheorem{definition}{Definition} %[chapter]
\newtheorem{claim}{Claim} %[chapter]
\newtheorem{proposition}{Proposition} %[chapter]
\newtheorem{cor}{Corollary} %[chapter]
\newtheorem{conj}{Conjecture} %[chapter]
\newtheorem{openq}{Open Question} %[chapter]

\newtheorem{remark}{Remark}[section] %[chapter]
\newtheorem{question}{Question}[section]

\newcommand{\quest}[1]{\begin{question}#1\end{question}}
\newcommand{\rmk}[1]{\begin{remark}#1\end{remark}}

%\newcommand{\aln}[1]{\begin{align*}#1\end{align*}}

\newenvironment{xlist}[1]{
  \begin{list}{}{
    \settowidth{\labelwidth}{#1}
    \setlength{\labelsep}{0.5cm}
    \setlength{\leftmargin}{\labelwidth}
    \addtolength{\leftmargin}{\labelsep}
    %\setlength{\rightmargin}{0pt}
    %\setlength{\parsep}{0.5ex plus0.2ex minus0.1ex}
    %\setlength{\itemsep}{0ex plus0.2ex}
    }
  }
{\end{list}}



%\usepackage{amsthm}

%\usepackage{ntheorem}

%\newenvironment{proof}{\noindent \emph{Proof:}\,}{\hfill $\blacksquare$}

\newenvironment{proofsketch}{\noindent \emph{Proof Sketch:}\,}{\hfill $\blacksquare$}

%\let\Oldproof\proof
\newenvironment{nproof}{\noindent \emph{Proof:}\,}{\hfill\IEEEQED}

%\newenvironment{proofof}[1]{\noindent \emph{Proof of #1:} \,}{\hfill $\blacksquare$}

\newenvironment{proofof}[1]{\noindent \emph{Proof of #1:} \,}{\hfill $\blacksquare$}

\newenvironment{proof_}[1]{\vspace{2mm} \noindent \emph{Proof #1:} \,}{\hfill\qed\\}

\renewcommand{\labelenumi}{(\alph{enumi})}

\renewcommand{\th}{^{\rm th}}

\newcounter{examplecounter}
\setcounter{examplecounter}{0}

\newenvironment{example}
{
%\stepcounter{theorem} {\vspace{4mm} \noindent \bf Example \arabic{thmcnt}.\arabic{theorem}.} \begin{it} \rm
\stepcounter{examplecounter} {\vspace{4mm} \noindent \bf Example \arabic{chapter}.\arabic{examplecounter}.} \begin{it} \rm
}
{
\end{it} \vspace{2mm}}

\newcommand{\aln}[1]{\begin{align*}#1\end{align*}}

\newcommand{\al}[1]{\begin{align}#1\end{align}}

%\newcommand{\quest}[1]{\noindent {\bf *** #1 ***}}

\newcommand{\Ns}{{\mathbf N}}

\def\Item$#1${\item $\displaystyle#1$
   \hfill\refstepcounter{equation}(\theequation)}

\setcounter{tocdepth}{1}


\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beas}{\begin{eqnarray*}}
\newcommand{\eeas}{\end{eqnarray*}}

